Gransformer: Transformer-based Graph Generation

Transformers have become widely used in various tasks, such as natural language processing and machine vision. This paper proposes Gransformer, an algorithm based on Transformer for generating graphs. We modify the Transformer encoder to exploit the structural information of the given graph. The attention mechanism is adapted to consider the presence or absence of edges between each pair of nodes. We also introduce a graph-based familiarity measure between node pairs that applies to both the attention and the positional encoding. This measure of familiarity is based on message-passing algorithms and contains structural information about the graph. Also, this measure is autoregressive, which allows our model to acquire the necessary conditional probabilities in a single forward pass. In the output layer, we also use a masked autoencoder for density estimation to efficiently model the sequential generation of dependent edges connected to each node. In addition, we propose a technique to prevent the model from generating isolated nodes without connection to preceding nodes by using BFS node orderings. We evaluate this method using synthetic and real-world datasets and compare it with related ones, including recurrent models and graph convolutional networks. Experimental results show that the proposed method performs comparatively to these methods.

==> bio.tex <==
 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pic/Khajehnejad.png}}]{Ahmad Khajehnejad}
	is a Ph.D. candidate at Sharif University of Technology. He received his B.Sc. and M.Sc. degrees in computer engineering from Sharif University of Technology, in 2010 and 2012, respectively. His research interests include learning probabilistic models for structured/distributed data.
    \end{IEEEbiography}
    \vspace{-0.6cm}
    \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pic/Madani.jpg}}]{Hatef Madani}
    received B.Sc. Degree in Computer Engineering from Kharazmi University of Tehran, in 2014. He also received the M.Sc degree in Computer Engineering from Sharif University of Technology, in 2018. He is interested in image processing and deep approaches in machine learning.
    \end{IEEEbiography}
    \vspace{-0.6cm}
    \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pic/Beigy.jpg}}]{Hamid Beigy}
	received the B.Sc. and M.Sc. degrees in computer engineering from the Shiraz university in Iran, in 1992 and 1995, respectively. He also received the Ph.D. degree in computer engineering from the Amirkabir university of technology, Iran, in 2004. Currently, he is an Associate Professor in department of computer engineering at the Sharif university of Technology, Tehran, Iran. His research interests include theoretical machine learning, large scale machine learning, and social networks.
    \end{IEEEbiography}

==> img/transformerAttentionOld.tex <==
\begin{tikzpicture}

\def \fs {\huge}

\begin{scope}[every node/.style={thick,draw, minimum width=2cm, minimum height=1cm, font=\fs}]
    \node (D1) at (0,0) {$h_1$};
    \node (D2) at (3,0) {$h_2$};
    \node (D3) at (9,0) {$h_{n-1}$};
    \node (D4) at (12,0) {$h_n$};
    \node (U1) at (0,7) {};
    \node (U2) at (3,7) {};
    \node (U3) at (9,7) {};
    \node (U4) at (12,7) {};
\end{scope}

\begin{scope}[every node/.style={font=\fs}]
    \node (Ddots) at (6,0) {\textbf{..........}};
    \node (Udots) at (6,7) {\textbf{..........}};
\end{scope}

\begin{scope}[every node/.style={thick,draw, minimum width=1.6cm, minimum height=1cm, font=\fs}]
    \node (V1) at (0,1) {$v_1$};
    \node (V2) at (3,1) {$v_2$};
    \node (V3) at (9,1) {$v_{n-1}$};
    \node (V4) at (12,1) {$v_n$};
\end{scope}


\begin{scope}[>={Stealth[black]},
              every edge/.style={draw=black,very thick}]
\draw [->] (V1) edge node {} (U2);
\path [->] (V2) edge node {} (U2);
\path [->] (V3) edge node {} (U2);
\path [->] (V4) edge node {} (U2);
\end{scope}


\begin{scope}[every node/.style={thick,circle, fill=white, font=\small}]
    \node (Att1) at (1.5,4) {$0.1$};
    \node (Att2) at (3,4) {$0.2$};
    \node (Att3) at (6,4) {$0.0$};
    \node (Att4) at (7.6,4) {$0.3$};
\end{scope}

\begin{scope}[every node/.style={thick, font=\fs}]
    \node (K1) at (-0.2, 2) {$k_1$};
    \node (K2) at (3.4, 2) {$k_2$};
    \node (K3) at (9.3, 2) {$k_{n-1}$};
    \node (K4) at (11.8, 2) {$k_n$};
    \node (Q2) at (3.4, 5.9) {$q_2$};
\end{scope}


\end{tikzpicture}
